Safraless Synthesis for Epistemic Temporal Specifications

In this paper we address the synthesis problem for specifications given in linear temporal single-agent epistemic logic, KLTL (or $KL_1$), over single-agent systems having imperfect information of the environment state. Van der Meyden and Vardi have shown that this problem is 2Exptime complete. However, their procedure relies on complex automata constructions that are notoriously resistant to efficient implementations as they use Safra-like determinization. We propose a "Safraless" synthesis procedure for a large fragment of KLTL. The construction transforms first the synthesis problem into the problem of checking emptiness for universal co-B\"{u}chi tree automata using an information-set construction. Then we build a safety game that can be solved using an antichain-based symbolic technique exploiting the structure of the underlying automata. The technique is implemented and applied to a couple of case studies.

==> proof7.tex <==
\begin{proof}
If $F'$ is winning for the system, then there exists a strategy $\lambda_1$ for the system from $F'$ that enforces the game to stay in the set $Safe$.
This means that there exists the strategy $\lambda_1$ such that all the paths from the states $(q,I)$ with $F'(q,I) \not = -1$ visit at most $B - \kappa(F',q)$ final states.

Then, since $\kappa(F,q) \subseteq \kappa(F',q)$, $\forall q$ and $\forall (q,I) \in Q, F(q,I) \leq F'(q,I)$ and because of the way the knowledge set $I$ is constructed using $Post_a(Y, o)$ (if $Y \subseteq Y'$, then $Post_a(Y,o) \subseteq Post_a(Y',o)$), there exists the strategy $\lambda_1$ such that all the paths from states $(q,I)$ with $F(q,I) \not = -1$ visit at most $B-\kappa(F,q)$ final states.

Therefore, there exists a strategy $\lambda_1$ from $F$ that enforces the game to stay in the set $Safe$ and, then, $F$ is winning for Player Ag. 

\end{proof}
